GazeTrak: Exploring Acoustic-based Eye Tracking on a Glass Frame

In this paper, we present GazeTrak, the first acoustic-based eye tracking system on glasses. Our system only needs one speaker and four microphones attached to each side of the glasses. These acoustic sensors capture the formations of the eyeballs and the surrounding areas by emitting encoded inaudible sound towards eyeballs and receiving the reflected signals. These reflected signals are further processed to calculate the echo profiles, which are fed to a customized deep learning pipeline to continuously infer the gaze position. In a user study with 20 participants, GazeTrak achieves an accuracy of 3.6{\deg} within the same remounting session and 4.9{\deg} across different sessions with a refreshing rate of 83.3 Hz and a power signature of 287.9 mW. Furthermore, we report the performance of our gaze tracking system fully implemented on an MCU with a low-power CNN accelerator (MAX78002). In this configuration, the system runs at up to 83.3 Hz and has a total power signature of 95.4 mW with a 30 Hz FPS.

==> 3_theory_of_operation.tex <==
\section{Theory of operation}
\label{Sec: Theory of operation}

Active acoustic sensing is based on affordable sensors (speakers and microphones), the sizes of which are relatively small. Previous research work has proved that active acoustic sensing with encoded signals is able to provide enough information to track subtle skin deformations such as facial expressions \cite{li2022eario,Gao2022sonicface}. As eyeballs are not perfectly spherical, when people rotate their eyes, the formation and shape of the eyeballs and the skin around them will be different and they may also be captured by a similar active acoustic sensing technique. In order to validate the feasibility of this sensing principle on tracking continuous gaze points, we attached an array of microphones and speakers along the inner side of a glass frame. The speakers generated encoded FMCW signals and the microphones captured the reflected signals. While wearing the glasses, one researcher tested the \gls{name} system by looking at different fixation points and making eye movements along different paths on the screen. Echo profiles (refer to Subsec. \ref{SubSec: FMCW}) corresponding to different fixation points and different movements are generated, which are shown in Fig. \ref{Fig: patterns}. From these traces we can see clear patterns for different eye positions. In this way, we believe that based on the active acoustic sensing principle, a well-designed system with acoustic sensors is capable of tracking continuous gaze points accurately.
